PixelDefend: Leveraging Generative Models to Understand and Defend against Adversarial Examples

Adversarial perturbations of normal images are usually imperceptible to humans, but they can seriously confuse state-of-the-art machine learning models. What makes them so special in the eyes of image classifiers? In this paper, we show empirically that adversarial examples mainly lie in the low probability regions of the training distribution, regardless of attack types and targeted models. Using statistical hypothesis testing, we find that modern neural density models are surprisingly good at detecting imperceptible image perturbations. Based on this discovery, we devised PixelDefend, a new approach that purifies a maliciously perturbed image by moving it back towards the distribution seen in the training data. The purified image is then run through an unmodified classifier, making our method agnostic to both the classifier and the attacking method. As a result, PixelDefend can be used to protect already deployed models and be combined with other model-specific defenses. Experiments show that our method greatly improves resilience across a wide variety of state-of-the-art attacking methods, increasing accuracy on the strongest attack from 63% to 84% for Fashion MNIST and from 32% to 70% for CIFAR-10.

==> intro-old-1.tex <==
\section{Introduction}

Recent work has shown that small modifications to the inputs of a machine learning model can cause the model to incorrectly classify the sample.  This is surprising because the necessary modifications are often imperceptable, or barely perceptable to humans.  Furthermore, these adversarial changes often cause the model to change from high confidence in the correct prediction to high confidence in the wrong prediction.  This problem is both practically important in the case of safty critical AI systems such as self-driving cars, but also theoretically important in providing insight in how to build models which generalize better.

{\bf Are adversarial examples really surprising:}  On the surface, the existence of such adversarial examples seems quite surprising.  We argue, however, that their existence should not be surprising, and is, in some sense, quite expected.  This assertion comes from one simple observation, {\em adversarial examples are not drawn from the same distribution as the training data}.
In particular, the natural images typically used to train image classifiers consists entirely of natural images.  And these natural images occupy only a very small manifold in the space of possible images.  The neural network is trained to maximize the probability of predicting the correct class for images in this manifold, without any constraints on the predictions it makes for images outside of this manifold.

The central idea of this paper is model the distribution of the training data using a modern generative image model, such as a PixelCNN, such that low-probability images under this model 


such that when images are low-probability under this model we cannot make any assumptions about the likely class of the examples.



allowing us to detec
Thus when images are low-p



and detect when images are outside of this distribution in order 


detect images which are outside of the manifold of the training images 


model 


the central idea of this paper is very simple.  use a generative model to learn the space of the training data, on which the classifier will do well and then do something else.



While the differences between images in 


subspace of the full space of possible images.


We know from the interpolation results of modern generative image models, that the support of various image classes overlap each other.  This forces the 

%yarin gal: bayesian neural networks -- adversarial examples
%https://arxiv.org/pdf/1703.02914.pdf

image classes smooth

Image classifiers are forced to choose a class distribution for every 


  The boundaries are 

the training data contains only clear natural images.  In contrast 

Even through the original image and the adversarial image differ by only a few pixels


%https://static.googleusercontent.com/media/research.google.com/en//pubs/archive/37065.pdf

Most of learning theory is based on the assumption that the test data and the training data are drawn from the same distribution.  In practice, however, it is typically difficult to obtain suffient labeled data from exactly the domain on which a system will be deployed.  This problem has been exacerbated recently, by the proliferation of deep learning models which require very large data sets for training. Furthermore, in reinforcement learning, exploration often leads to new part of the state space significantly different from those on which the existing policy has been trained.  Adversarial examples are an extreme example of mismatch between the training and test distribution, where the test data differs from the training data in the worst possible way for the model.  Thus the study of these examples can give us insights into how to build models with better generalization capabilities.

{\bf Correctly calibrated confidence:}
Existing work on confidence estimates for deep learning has focused on {\em Bayesian deep learning}, which puts a prior over the parameters $\theta$, such that at test time, the prediction is chosen by maximizing the expected probability over all choices of $\theta$.  While theoretically satisfying,

Basic problem is that $p(x|\theta)==p(x)$, and so we can easily change the generative model into a discriminative one which does not depend on $\theta$


Basic pitch:
- Existing work has focused on adversarial training.  We employ a different technique. Instead of retraining the underlying model, we project the example onto the training distribution, and then classify it according to the underlying model.



{\bf Correctly calibrated confidence:}
Existing work on confidence estimates for deep learning has focused on {\em Bayesian deep learning}, which puts a prior over the parameters $\theta$, such that for input data $X$, and output labels $Y$:
\begin{align}
  p(\theta|\boldsymbol{X},\boldsymbol{Y})=\frac{p(\boldsymbol{Y}|\boldsymbol{X},\theta)p(\theta)}{p(\boldsymbol{Y}|\boldsymbol{X})}\\
  p(\theta|\boldsymbol{X},\boldsymbol{Y})=\frac{p(\boldsymbol{Y},\boldsymbol{X}|\theta)p(\theta)}{p(\boldsymbol{Y},\boldsymbol{X})}\\
  p(\theta|\boldsymbol{X},\boldsymbol{Y})=\frac{p(\boldsymbol{Y}|\boldsymbol{X},\theta)p(\boldsymbol{X}|\theta)p(\theta)}{p(\boldsymbol{Y}|\boldsymbol{X})p(\boldsymbol{X})}\\
\end{align}
\begin{align}
  p(\theta|\boldsymbol{X},\boldsymbol{Y})=\frac{p(\boldsymbol{Y}|\boldsymbol{X},\theta)p(\theta)}{\int p(\boldsymbol{Y}|\boldsymbol{X},\theta)p(\theta)d\theta}\\
  p(\theta|\boldsymbol{X},\boldsymbol{Y})=\frac{p(\boldsymbol{Y},\boldsymbol{X}|\theta)p(\theta)}{\int p(\boldsymbol{Y},\boldsymbol{X}|\theta)p(\theta)d\theta}\\
  p(\theta|\boldsymbol{X},\boldsymbol{Y})=\frac{p(\boldsymbol{Y}|\boldsymbol{X},\theta)p(\boldsymbol{X}|\theta)p(\theta)}{\int p(\boldsymbol{Y}|\boldsymbol{X},\theta')p(\boldsymbol{X}|\theta')p(\theta')d\theta'}\\
\end{align}
At test time, given a novel input $x'$, output $y'$ is chosen by minimizing the expected loss over all choices of parameter values, as follows:
\begin{align}
p(y'|x',\boldsymbol{X},\boldsymbol{Y})=\int p(y'|x',\theta)p(\theta|\boldsymbol{X},\boldsymbol{Y})d\theta
\end{align}





and in particular the framework of empirical risk minimization.  Consider for example, data $x$, labels, $y$, and a model $h(x)$ which predicts a label for a given data sample.  Empirical risk minimization finds the model $h$ in some space of possible models $H$ which minimizes the risk, $R(h)$, defined as follows:
%\begin{align}
%  R(h)=\frac{1}{n}\sum_{i=1}^{n}I(h(x_i),y_i)
%\end{align}


*****Make the argument that once you have enough data then you will have a high probability on theta even though far away things aren't that likely.
*********

which typically puts some kind of generic gaussian prior on the parameters.

Two possible arguments:
1.  Different distributions:
-

2.  The idea of priors over parameters is not able to appropriately capture our understanding

Empirical Risk Minimization assumes that the training and test distributions of x,y are the same, i.e. they are drawn from the same distribtuion

What about Yarin Gal's stuff, or bayesian deep learning in general?




Basic argument:
- 




which has mostly focused on situations where the training and test data are drawn from the same distribtion.  For example, ~\cite{gal} focuses on the distinction between epistemic uncertainly, the uncertainty over the many possible models that fit the data equally well, and aleatoric uncertainty which comes from measurement noise, or stocasticity in the underlying domain.  These are both measures of the training data, however.  We argue that there's a third type of uncertainty, which we call data uncertainty.  


and ignore the possibly mismatch between the training and test distribution.  We argue that there


Howev

A first step in handling adversarial examples is ensure that even if we cannot correctly classify them, we are at least able to report low-confidence for them.

In many applications, it is sufficient to merely detect test samples which are outside of the training distribution, to either flag them for human intervention or skip them entirely~\cite{XXX}.  



systems are often trained on data from one domain

systems are typically trained on data from one domain, and then use


\noindent{\bf How to handle examples outside the training distribution:}    However, in many applications, human intervenction is not an option, and the system must make a decision for all samples.  In this case,   


Most of the work up until now has focused on 

such examples are not surprising given that the adversarial examples do not come from the same distribution as the training data.  In fact, we argue that in general it's 

the models often change from high confidence in one sample, to high confidence in another sample.



Outline:
1.  Intro to adversarial examples. Small changes cause major classification errors
2.  bold no indent title:  Something about adversarial examples are not surprising -- basically confidence is just wrong if the data does not come from the training distribution -- trained on different subsets of the data, same problem, so there's a general problem here
3.  fix examples by projecting them back

Contributions:
xxx
xxx
xxx





Main Points:

Adversarial examples are not surprising because 




Possible ideas for pitch:
1. questioning empirical risk minimization
  - I don't think I understand this argument
2. existing defense mechanisms don't work against the state of the art attack mechanisms 
3.  Adversarial examples are not surprising:
- outside the training manifold
- we can detect this with pixelcnn

The idea of known unknows vs. unknown unknowns:
- make the argument that in general confidence in neural networks is broken
- idea Bayesian or otherwise

Generalization does not imply robustness

adversarial examples are known unknowns (we know that they're outside the training distribution)


Yang's ideas:
* Imperceptible perturbations (whether adversarial or not) result in images clearly outside the training distribution in the eye of generative models (PixelCNN and Real NVP).
* Since those perturbed images are outside the training distribution, there is no guarantee for classifiers to be robust to them. Good generalization doesn't imply robustness.
* Some models are clearly robust to random perturbations. This is not due to the learning procedure. In other words, their predictions will be robust no matter what values their parameters have
* Adversarial examples can fool classifiers to output wrong labels with high confidence because the classifier's confidence is on known unknowns.
* For a classifier to develop a correct notion of uncertainty, it is necessary to model unknown unknowns, which must involve training a generative model separately or modifying the training objective.
* If the classifier is forced to give a prediction on unknown unknown, the best bet is to first convert it to known unknown (keeping the labels) and then do prediction.

